Autonomous Systems' Safety Cases for use in UK Nuclear Environments

An overview of the process to develop a safety case for an autonomous robot deployment on a nuclear site in the UK is described and a safety case for a hypothetical robot incorporating AI is presented. This forms a first step towards a deployment, showing what is possible now and what may be possible with development of tools. It forms the basis for further discussion between nuclear site licensees, the Office for Nuclear Regulation (ONR), industry and academia.

==> eptcsdata.tex <==
\providecommand{\firstpage}{83}
\providecommand{\publicationstatus}{A. Ferrando, R.C. Cardoso (Eds.): Third Workshop on\\ Agents and Robots for reliable Engineered Autonomy 2023 (AREA'23)\\
EPTCS 391, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.391.10}{10.4204/EPTCS.391.10}}
\pdfoutput=1

